Emergent superconductivity upon disordering a charge density wave ground state

We explore the interplay of a charge density wave (CDW) order and s-wave superconductivity (sSC) in a disordered system. Recent experiments on 1T-TiSe_2, where the pristine sample has a commensurate CDW order and the superconductivity appears upon copper intercalation, motivates our study. Starting with an extended Hubbard model, with parameters which yield a CDW ground state within Hartree-Fock-Bogoliubov formalism in pure systems, we show that the addition of disorder quickly wipes out the global charge order by disrupting periodic modulation of density at some (low) strength of disorder. Along with this, the subdominant superconducting order emerges in regions that spatially anti-correlates with islands of strong local CDW order. The short-range density modulations, however, continue to persist and show discernible effects up to a larger disorder strength. The local CDW puddles reduce in size with increasing disorder and they finally lose their relevance in effecting the properties of the system. Our results have strong implications for the experimental phase diagram of transition metal dichalcogenides.

==> References <==

@article{ThUnconvSC,
  title = {Phenomenological theory of unconventional superconductivity},
  author = {Sigrist, Manfred and Ueda, Kazuo},
  journal = {Rev. Mod. Phys.},
  volume = {63},
  issue = {2},
  pages = {239--311},
  numpages = {0},
  year = {1991},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.63.239},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.63.239}
}
@article {Norman196,
	author = {Norman, Michael R.},
	title = {The Challenge of Unconventional Superconductivity},
	volume = {332},
	number = {6026},
	pages = {196--200},
	year = {2011},
	doi = {10.1126/science.1200181},
	publisher = {American Association for the Advancement of Science},
	URL = {http://science.sciencemag.org/content/332/6026/196},
	eprint = {http://science.sciencemag.org/content/332/6026/196.full.pdf},
	journal = {Science}
}

@Article{CVarma,
author={Varma, Chandra},
title={Mind the pseudogap},
journal={Nature},
year={2010},
month={Nov},
day={10},
publisher={Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved. SN  -},
volume={468},
pages={184 EP  -},
url={http://dx.doi.org/10.1038/468184a}
}


@article{Dagotto,
  title = {Correlated electrons in high-temperature superconductors},
  author = {Dagotto, Elbio},
  journal = {Rev. Mod. Phys.},
  volume = {66},
  issue = {3},
  pages = {763--840},
  numpages = {0},
  year = {1994},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.66.763},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.66.763}
}


@book{PdGbook,
  title={Superconductivity of Metals and Alloys},
  author={De Gennes, P.G.},
  lccn={lc65017013},
  series={Frontiers in physics},
  url={https://books.google.co.in/books?id=KtJEAAAAIAAJ},
  year={1966},
  publisher={Benjamin}
}

@article{SWZ,
  title = {Insulator, metal, or superconductor: The criteria},
  author = {Scalapino, Douglas J. and White, Steven R. and Zhang, Shoucheng},
  journal = {Phys. Rev. B},
  volume = {47},
  issue = {13},
  pages = {7995--8007},
  numpages = {0},
  year = {1993},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.47.7995},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.47.7995}
}

@book{DWinSolids,
  title={Density Waves in Solids},
  author={George Gr{\"u}ner},
  isbn={9780201626544},
  lccn={93032362},
  series={Advanced book program: Addison-Wesley},
  url={https://books.google.co.in/books?id=6GksAAAAYAAJ},
  year={2000},
  publisher={Perseus Books Group}
}

@article{PWA,
  title = {Absence of Diffusion in Certain Random Lattices},
  author = {Anderson, P. W.},
  journal = {Phys. Rev.},
  volume = {109},
  issue = {5},
  pages = {1492--1505},
  numpages = {0},
  year = {1958},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.109.1492},
  url = {https://link.aps.org/doi/10.1103/PhysRev.109.1492}
}

@article{AndTheo,
title = "Theory of dirty superconductors",
journal = "Journal of Physics and Chemistry of Solids",
volume = "11",
number = "1",
pages = "26 - 30",
year = "1959",
issn = "0022-3697",
doi = "https://doi.org/10.1016/0022-3697(59)90036-8",
url = "http://www.sciencedirect.com/science/article/pii/0022369759900368",
author = "P.W. Anderson"
}


%-------------------HTSc and AFM
@Article{Lu2014,
author={Lu, X. F.
and Wang, N. Z.
and Wu, H.
and Wu, Y. P.
and Zhao, D.
and Zeng, X. Z.
and Luo, X. G.
and Wu, T.
and Bao, W.
and Zhang, G. H.
and Huang, F. Q.
and Huang, Q. Z.
and Chen, X. H.},
title={Coexistence of superconductivity and antiferromagnetism in (Li0.8Fe0.2)OHFeSe},
journal={Nature Materials},
year={2014},
month={Dec},
day={15},
publisher={Nature Publishing Group SN  -},
volume={14},
pages={325 EP  -},
note={Article},
url={http://dx.doi.org/10.1038/nmat4155}
}

	

@article {Sachdev1510,
	author = {Sachdev, Subir},
	title = {Entangling Superconductivity and Antiferromagnetism},
	volume = {336},
	number = {6088},
	pages = {1510--1511},
	year = {2012},
	doi = {10.1126/science.1223586},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/336/6088/1510},
	eprint = {http://science.sciencemag.org/content/336/6088/1510.full.pdf},
	journal = {Science}
}

@article{So5RMP,
  title = {$\mathit{SO}(5)$},
  author = {Demler, Eugene and Hanke, Werner and Zhang, Shou-Cheng},
  journal = {Rev. Mod. Phys.},
  volume = {76},
  issue = {3},
  pages = {909--974},
  numpages = {0},
  year = {2004},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.76.909},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.76.909}
}

%------------------Orbital Order in Ruthnates--------------------------------
@article{Ruth0,
  title = {Tunneling magnetoresistance and quantum oscillations in bilayered ${\mathrm{Ca}}_{3}{\mathrm{Ru}}_{2}{\mathrm{O}}_{7}$},
  author = {Cao, G. and Balicas, L. and Xin, Y. and Dagotto, E. and Crow, J. E. and Nelson, C. S. and Agterberg, D. F.},
  journal = {Phys. Rev. B},
  volume = {67},
  issue = {6},
  pages = {060406},
  numpages = {4},
  year = {2003},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.67.060406},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.67.060406}
}

@article{Ruth1,
  title = {Quasi-Two-Dimensional Mott Transition System ${\mathrm{Ca}}_{2\ensuremath{-}\mathit{x}}{\mathrm{Sr}}_{\mathit{x}}{\mathrm{RuO}}_{4}$},
  author = {Nakatsuji, S. and Maeno, Y.},
  journal = {Phys. Rev. Lett.},
  volume = {84},
  issue = {12},
  pages = {2666--2669},
  numpages = {0},
  year = {2000},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.84.2666},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.84.2666}
}

@article{Ruth2,
  title = {Pressure-Tuned Collapse of the Mott-Like State in ${\mathrm{C}\mathrm{a}}_{n+1}{\mathrm{R}\mathrm{u}}_{n}{\mathrm{O}}_{3n+1}$ ($n=1,2$): Raman Spectroscopic Studies},
  author = {Snow, C. S. and Cooper, S. L. and Cao, G. and Crow, J. E. and Fukazawa, H. and Nakatsuji, S. and Maeno, Y.},
  journal = {Phys. Rev. Lett.},
  volume = {89},
  issue = {22},
  pages = {226401},
  numpages = {4},
  year = {2002},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.89.226401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.89.226401}
}


%---------------------Experiments on 1T-TiSe2--------------------------------------
@Article{Cava0,
author={Morosan, E.
and Zandbergen, H. W.
and Dennis, B. S.
and Bos, J. W. G.
and Onose, Y.
and Klimczuk, T.
and Ramirez, A. P.
and Ong, N. P.
and Cava, R. J.},
title={Superconductivity in CuxTiSe2},
journal={Nature Physics},
year={2006},
month={Jul},
day={23},
publisher={Nature Publishing Group SN  -},
volume={2},
pages={544 EP  -},
note={Article},
url={http://dx.doi.org/10.1038/nphys360}
}

@article{Cava1,
  title = {Anisotropic properties of the layered superconductor ${\mathrm{Cu}}_{0.07}\mathrm{Ti}{\mathrm{Se}}_{2}$},
  author = {Morosan, E. and Li, Lu and Ong, N. P. and Cava, R. J.},
  journal = {Phys. Rev. B},
  volume = {75},
  issue = {10},
  pages = {104505},
  numpages = {5},
  year = {2007},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.75.104505},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.75.104505}
}

@article{Cava2,
  title = {Quantum and Classical Mode Softening Near the Charge-Density-Wave\char21{}Superconductor Transition of ${\mathrm{Cu}}_{x}{\mathrm{TiSe}}_{2}$},
  author = {Barath, H. and Kim, M. and Karpus, J. F. and Cooper, S. L. and Abbamonte, P. and Fradkin, E. and Morosan, E. and Cava, R. J.},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {10},
  pages = {106402},
  numpages = {4},
  year = {2008},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.100.106402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.100.106402}
}

@article{MonolayTiSe2,
  title = {Stable charge density wave phase in a $1T\char21{}{\mathrm{TiSe}}_{2}$ monolayer},
  author = {Singh, Bahadur and Hsu, Chuang-Han and Tsai, Wei-Feng and Pereira, Vitor M. and Lin, Hsin},
  journal = {Phys. Rev. B},
  volume = {95},
  issue = {24},
  pages = {245136},
  numpages = {7},
  year = {2017},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.95.245136},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.95.245136}
}

@article{Maydop,
  title = {Charge-Density-Wave Phase of $1T\mathrm{\text{\ensuremath{-}}}{\mathrm{TiSe}}_{2}$: The Influence of Conduction Band Population},
  author = {May, Matthias M. and Brabetz, Christine and Janowitz, Christoph and Manzke, Recardo},
  journal = {Phys. Rev. Lett.},
  volume = {107},
  issue = {17},
  pages = {176405},
  numpages = {4},
  year = {2011},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.107.176405},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.107.176405}
}

@article{ChiralCDW,
  title = {Chiral Phase Transition in Charge Ordered $1T\mathrm{\text{\ensuremath{-}}}{\mathrm{TiSe}}_{2}$},
  author = {Castellan, John-Paul and Rosenkranz, Stephan and Osborn, Ray and Li, Qing'an and Gray, K. E. and Luo, X. and Welp, U. and Karapetrov, Goran and Ruff, J. P. C. and van Wezel, Jasper},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {19},
  pages = {196404},
  numpages = {5},
  year = {2013},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.196404},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.196404}
}

@article{DisorderTiSe2,
  title = {Point-contact tunneling spectroscopy measurement of ${\mathrm{Cu}}_{x}{\mathrm{TiSe}}_{2}$: Disorder-enhanced Coulomb effects},
  author = {Luna, Katherine and Wu, Phillip M. and Chen, Justin S. and Morosan, Emilia and Beasley, Malcolm R.},
  journal = {Phys. Rev. B},
  volume = {91},
  issue = {9},
  pages = {094509},
  numpages = {4},
  year = {2015},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.91.094509},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.91.094509}
}

@article{DefectsTiSe2,
  title = {Doping Nature of Native Defects in $1T\text{\ensuremath{-}}{\mathrm{TiSe}}_{2}$},
  author = {Hildebrand, B. and Didiot, C. and Novello, A. M. and Monney, G. and Scarfato, A. and Ubaldini, A. and Berger, H. and Bowler, D. R. and Renner, C. and Aebi, P.},
  journal = {Phys. Rev. Lett.},
  volume = {112},
  issue = {19},
  pages = {197001},
  numpages = {5},
  year = {2014},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.112.197001},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.112.197001}
}

@article{FSpocket,
  title = {Emergence of Fermi Pockets in a New Excitonic Charge-Density-Wave Melted Superconductor},
  author = {Qian, D. and Hsieh, D. and Wray, L. and Morosan, E. and Wang, N. L. and Xia, Y. and Cava, R. J. and Hasan, M. Z.},
  journal = {Phys. Rev. Lett.},
  volume = {98},
  issue = {11},
  pages = {117007},
  numpages = {4},
  year = {2007},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.98.117007},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.98.117007}
}

@article{IavaroneCuxTiSe2,
  title = {Evolution of the charge density wave state in Cu${}_{x}$TiSe${}_{2}$},
  author = {Iavarone, M. and Di Capua, R. and Zhang, X. and Golalikhani, M. and Moore, S. A. and Karapetrov, G.},
  journal = {Phys. Rev. B},
  volume = {85},
  issue = {15},
  pages = {155103},
  numpages = {6},
  year = {2012},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.85.155103},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.85.155103}
}

@article{Abbamonte,
  title = {Observation of a Charge Density Wave Incommensuration Near the Superconducting Dome in ${\mathrm{Cu}}_{x}{\mathrm{TiSe}}_{2}$},
  author = {Kogar, A. and de la Pena, G. A. and Lee, Sangjun and Fang, Y. and Sun, S. X.-L. and Lioi, D. B. and Karapetrov, G. and Finkelstein, K. D. and Ruff, J. P. C. and Abbamonte, P. and Rosenkranz, S.},
  journal = {Phys. Rev. Lett.},
  volume = {118},
  issue = {2},
  pages = {027002},
  numpages = {5},
  year = {2017},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.118.027002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.027002}
}

@article{YanSTM,
  title = {Influence of Domain Walls in the Incommensurate Charge Density Wave State of Cu Intercalated $1T\text{\ensuremath{-}}{\mathrm{TiSe}}_{2}$},
  author = {Yan, Shichao and Iaia, Davide and Morosan, Emilia and Fradkin, Eduardo and Abbamonte, Peter and Madhavan, Vidya},
  journal = {Phys. Rev. Lett.},
  volume = {118},
  issue = {10},
  pages = {106405},
  numpages = {5},
  year = {2017},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.118.106405},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.106405}
}

@Article{PressureTiSe2,
author={Joe, Y. I.
and Chen, X. M.
and Ghaemi, P.
and Finkelstein, K. D.
and de la Pe{\~n}a, G. A.
and Gan, Y.
and Lee, J. C. T.
and Yuan, S.
and Geck, J.
and MacDougall, G. J.
and Chiang, T. C.
and Cooper, S. L.
and Fradkin, E.
and Abbamonte, P.},
title={Emergence of charge density wave domain walls above the superconducting dome in 1T-TiSe2},
journal={Nature Physics},
year={2014},
month={Apr},
day={06},
publisher={Nature Publishing Group SN  -},
volume={10},
pages={421 EP  -},
url={http://dx.doi.org/10.1038/nphys2935}
}

@article{CvforCuxTiSe2,
  title = {Heat capacity of single-crystal Cu${}_{x}$TiSe${}_{2}$ superconductors},
  author = {Ka\ifmmode \check{c}\else \v{c}\fi{}mar\ifmmode \check{c}\else \v{c}\fi{}\'{\i}k, J. and Pribulov\'a, Z. and Pal'uchov\'a, V. and Szab\'o, P. and Husan\'{\i}kov\'a, P. and Karapetrov, G. and Samuely, P.},
  journal = {Phys. Rev. B},
  volume = {88},
  issue = {2},
  pages = {020507},
  numpages = {5},
  year = {2013},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.88.020507},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.88.020507}
}

@article{TiDop,
  title = {Local resilience of the $1T\text{\ensuremath{-}}{\mathrm{TiSe}}_{2}$ charge density wave to Ti self-doping},
  author = {Hildebrand, B. and Jaouen, T. and Didiot, C. and Razzoli, E. and Monney, G. and Mottas, M.-L. and Vanini, F. and Barreteau, C. and Ubaldini, A. and Giannini, E. and Berger, H. and Bowler, D. R. and Aebi, P.},
  journal = {Phys. Rev. B},
  volume = {95},
  issue = {8},
  pages = {081104},
  numpages = {5},
  year = {2017},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.95.081104},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.95.081104}
}

@article{MEinCuxTiSe2,
  title = {Observation of a transverse Meissner effect in ${\mathrm{Cu}}_{x}{\mathrm{TiSe}}_{2}$ single crystals},
  author = {Medveck\'a, Z. and Klein, T. and Cambel, V. and \ifmmode \check{S}\else \v{S}\fi{}olt\'ys, J. and Karapetrov, G. and Levy-Bertrand, F. and Michon, B. and Marcenat, C. and Pribulov\'a, Z. and Samuely, P.},
  journal = {Phys. Rev. B},
  volume = {93},
  issue = {10},
  pages = {100501},
  numpages = {5},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.93.100501},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.93.100501}
}

@article{2gap,
  title = {Possible evidence of a two-gap structure for the ${\text{Cu}}_{x}{\text{TiSe}}_{2}$ superconductor},
  author = {Zaberchik, Moran and Chashka, Khanan and Patlgan, Larisa and Maniv, Ariel and Baines, Chris and King, Philip and Kanigel, Amit},
  journal = {Phys. Rev. B},
  volume = {81},
  issue = {22},
  pages = {220505},
  numpages = {4},
  year = {2010},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.81.220505},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.81.220505}
}

@article{PressurePRL,
  title = {Pressure Induced Superconductivity in Pristine $1T\mathrm{\text{\ensuremath{-}}}{\mathrm{TiSe}}_{2}$},
  author = {Kusmartseva, A. F. and Sipos, B. and Berger, H. and Forr\'o, L. and Tuti\ifmmode \check{s}\else \v{s}\fi{}, E.},
  journal = {Phys. Rev. Lett.},
  volume = {103},
  issue = {23},
  pages = {236401},
  numpages = {4},
  year = {2009},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.103.236401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.103.236401}
}

@article{ProbTransCuTiSe2,
  title = {Probing the superconducting ground state near the charge density wave phase transition in ${\text{Cu}}_{0.06}{\text{TiSe}}_{2}$},
  author = {Hillier, A. D. and Manuel, P. and Adroja, D. T. and Taylor, J. W. and Azad, A. K. and Irvine, J. T. S.},
  journal = {Phys. Rev. B},
  volume = {81},
  issue = {9},
  pages = {092507},
  numpages = {4},
  year = {2010},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.81.092507},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.81.092507}
}

@article{Pddop,
  title = {Multiple electronic transitions and superconductivity in ${\text{Pd}}_{x}{\text{TiSe}}_{2}$},
  author = {Morosan, E. and Wagner, K. E. and Zhao, Liang L. and Hor, Y. and Williams, A. J. and Tao, J. and Zhu, Y. and Cava, R. J.},
  journal = {Phys. Rev. B},
  volume = {81},
  issue = {9},
  pages = {094524},
  numpages = {5},
  year = {2010},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.81.094524},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.81.094524}
}

@article{QMCDW,
  title = {Quantum Melting of the Charge-Density-Wave State in $1T\mathrm{\text{\ensuremath{-}}}{\mathrm{T}\mathrm{i}\mathrm{S}\mathrm{e}}_{2}$},
  author = {Snow, C. S. and Karpus, J. F. and Cooper, S. L. and Kidd, T. E. and Chiang, T.-C.},
  journal = {Phys. Rev. Lett.},
  volume = {91},
  issue = {13},
  pages = {136402},
  numpages = {4},
  year = {2003},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.91.136402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.91.136402}
}

@article{CDWpud0,
  title = {Stripe and Short Range Order in the Charge Density Wave of $1T\text{\ensuremath{-}}{\mathrm{Cu}}_{x}{\mathrm{TiSe}}_{2}$},
  author = {Novello, A. M. and Spera, M. and Scarfato, A. and Ubaldini, A. and Giannini, E. and Bowler, D. R. and Renner, Ch.},
  journal = {Phys. Rev. Lett.},
  volume = {118},
  issue = {1},
  pages = {017002},
  numpages = {5},
  year = {2017},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.118.017002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.017002}
}

@article{TiSTM,
  title = {Short-range phase coherence and origin of the $1T\ensuremath{-}{\mathrm{TiSe}}_{2}$ charge density wave},
  author = {Hildebrand, B. and Jaouen, T. and Didiot, C. and Razzoli, E. and Monney, G. and Mottas, M.-L. and Ubaldini, A. and Berger, H. and Barreteau, C. and Beck, H. and Bowler, D. R. and Aebi, P.},
  journal = {Phys. Rev. B},
  volume = {93},
  issue = {12},
  pages = {125140},
  numpages = {5},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.93.125140},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.93.125140}
}

@article{xrayTiSe2,
  title = {Superconductivity and hybrid soft modes in $\mathrm{Ti}{\mathrm{Se}}_{2}$},
  author = {Maschek, M. and Rosenkranz, S. and Hott, R. and Heid, R. and Merz, Michael and Zocco, D. A. and Said, A. H. and Alatas, A. and Karapetrov, G. and Zhu, Shan and van Wezel, Jasper and Weber, F.},
  journal = {Phys. Rev. B},
  volume = {94},
  issue = {21},
  pages = {214507},
  numpages = {10},
  year = {2016},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.94.214507},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.94.214507}
}

@article{BussmannPRB,
  title = {Suppression of charge-density formation in ${\text{TiSe}}_{2}$ by Cu doping},
  author = {Bussmann-Holder, A. and Bishop, A. R.},
  journal = {Phys. Rev. B},
  volume = {79},
  issue = {2},
  pages = {024302},
  numpages = {4},
  year = {2009},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.79.024302},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.79.024302}
}

@article{transportCuxTiSe2,
  title = {Transport properties of single-crystalline ${\mathrm{Cu}}_{x}\mathrm{Ti}{\mathrm{Se}}_{2}$ $(0.015\ensuremath{\leqslant}x\ensuremath{\leqslant}0.110)$},
  author = {Wu, G. and Yang, H. X. and Zhao, L. and Luo, X. G. and Wu, T. and Wang, G. Y. and Chen, X. H.},
  journal = {Phys. Rev. B},
  volume = {76},
  issue = {2},
  pages = {024513},
  numpages = {5},
  year = {2007},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.76.024513},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.76.024513}
}

@article{Samuelymagnetic,
  title = {Magnetic and thermodynamic properties of ${\mathrm{Cu}}_{x}{\mathrm{TiSe}}_{2}$ single crystals},
  author = {Pribulov\'a, Z. and Medveck\'a, Z. and Ka\ifmmode \check{c}\else \v{c}\fi{}mar\ifmmode \check{c}\else \v{c}\fi{}\'{\i}k, J. and Komanick\'y, V. and Klein, T. and Rodi\`ere, P. and Levy-Bertrand, F. and Michon, B. and Marcenat, C. and Husan\'{\i}kov\'a, P. and Cambel, V. and \ifmmode \check{S}\else \v{S}\fi{}olt\'ys, J. and Karapetrov, G. and Borisenko, S. and Evtushinsky, D. and Berger, H. and Samuely, P.},
  journal = {Phys. Rev. B},
  volume = {95},
  issue = {17},
  pages = {174512},
  numpages = {8},
  year = {2017},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.95.174512},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.95.174512}
}

@article{VortexTiSe2,
  title = {Magnetization properties and vortex phase diagram of Cu${}_{x}$TiSe${}_{2}$ single crystals},
  author = {Husan\'{\i}kov\'a, P. and Fedor, J. and D\'erer, J. and \ifmmode \check{S}\else \v{S}\fi{}olt\'ys, J. and Cambel, V. and Iavarone, M. and May, S. J. and Karapetrov, G.},
  journal = {Phys. Rev. B},
  volume = {88},
  issue = {17},
  pages = {174501},
  numpages = {5},
  year = {2013},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.88.174501},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.88.174501}
}

@article{ARPESCuxTiSe2,
  title = {Evolution of the Electronic Structure of $1T\mathrm{\text{\ensuremath{-}}}{\mathrm{Cu}}_{x}{\mathrm{TiSe}}_{2}$},
  author = {Zhao, J. F. and Ou, H. W. and Wu, G. and Xie, B. P. and Zhang, Y. and Shen, D. W. and Wei, J. and Yang, L. X. and Dong, J. K. and Arita, M. and Namatame, H. and Taniguchi, M. and Chen, X. H. and Feng, D. L.},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {14},
  pages = {146401},
  numpages = {4},
  year = {2007},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.99.146401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.99.146401}
}

@article{CDWpud1,
  title = {Short-range phase coherence and origin of the $1T\ensuremath{-}{\mathrm{TiSe}}_{2}$ charge density wave},
  author = {Hildebrand, B. and Jaouen, T. and Didiot, C. and Razzoli, E. and Monney, G. and Mottas, M.-L. and Ubaldini, A. and Berger, H. and Barreteau, C. and Beck, H. and Bowler, D. R. and Aebi, P.},
  journal = {Phys. Rev. B},
  volume = {93},
  issue = {12},
  pages = {125140},
  numpages = {5},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.93.125140},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.93.125140}
}

@Article{Porer2014,
author={Porer, M.
and Leierseder, U.
and M{\'e}nard, J.-M.
and Dachraoui, H.
and Mouchliadis, L.
and Perakis, I. E.
and Heinzmann, U.
and Demsar, J.
and Rossnagel, K.
and Huber, R.},
title={Non-thermal separation of electronic and structural orders in a persisting charge density wave},
journal={Nature Materials},
year={2014},
month={Jul},
day={20},
publisher={Nature Publishing Group SN  -},
volume={13},
pages={857 EP  -},
url={http://dx.doi.org/10.1038/nmat4042}
}

%------------------------Theory TMDs---------------------------
@article{ctoICDW,
author = { Kazuo Nakanishi and  Hiroyuki Shiba},
title = {Domain-like Incommensurate Charge-Density-Wave States and the First-Order Incommensurate-Commensurate Transitions in Layered Tantalum Dichalcogenides. I. 1T-Polytype},
journal = {Journal of the Physical Society of Japan},
volume = {43},
number = {6},
pages = {1839-1847},
year = {1977},
doi = {10.1143/JPSJ.43.1839},

URL = { 
        https://doi.org/10.1143/JPSJ.43.1839
    
},
eprint = { 
        https://doi.org/10.1143/JPSJ.43.1839
    
}}

@article{McMillan0,
  title = {Landau theory of charge-density waves in transition-metal dichalcogenides},
  author = {McMillan, W. L.},
  journal = {Phys. Rev. B},
  volume = {12},
  issue = {4},
  pages = {1187--1196},
  numpages = {0},
  year = {1975},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.12.1187},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.12.1187}
}

@article{McMillan1,
  title = {Theory of discommensurations and the commensurate-incommensurate charge-density-wave phase transition},
  author = {McMillan, W. L.},
  journal = {Phys. Rev. B},
  volume = {14},
  issue = {4},
  pages = {1496--1502},
  numpages = {0},
  year = {1976},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.14.1496},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.14.1496}
}

@article{Littlewood0,
  title = {Impurity pinning of discommensurations in charge-density waves},
  author = {Rice, T. M. and Whitehouse, S. and Littlewood, P.},
  journal = {Phys. Rev. B},
  volume = {24},
  issue = {5},
  pages = {2751--2759},
  numpages = {0},
  year = {1981},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.24.2751},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.24.2751}
}

@article{DFTTiSe2,
  title = {Electronic structure of superconducting copper intercalated transition metal dichalcogenides: First-principles calculations},
  author = {Jishi, R. A. and Alyahyaei, H. M.},
  journal = {Phys. Rev. B},
  volume = {78},
  issue = {14},
  pages = {144516},
  numpages = {7},
  year = {2008},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.78.144516},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.78.144516}
}

@article{IntbwCuDFT,
  title = {Interactions between copper and transition metal dichalcogenides: A density functional theory study},
  author = {Helfrecht, Benjamin A. and Guzman, David M. and Onofrio, Nicolas and Strachan, Alejandro H.},
  journal = {Phys. Rev. Materials},
  volume = {1},
  issue = {3},
  pages = {034001},
  numpages = {13},
  year = {2017},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevMaterials.1.034001},
  url = {https://link.aps.org/doi/10.1103/PhysRevMaterials.1.034001}
}

@article{OrginDFT,
  title = {Origin of the charge density wave in 1$T$-TiSe${}_{2}$},
  author = {Zhu, Zhiyong and Cheng, Yingchun and Schwingenschl\"ogl, Udo},
  journal = {Phys. Rev. B},
  volume = {85},
  issue = {24},
  pages = {245133},
  numpages = {4},
  year = {2012},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.85.245133},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.85.245133}
}

@article{Rice0,
  title = {New Mechanism for a Charge-Density-Wave Instability},
  author = {Rice, T. M. and Scott, G. K.},
  journal = {Phys. Rev. Lett.},
  volume = {35},
  issue = {2},
  pages = {120--123},
  numpages = {0},
  year = {1975},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.35.120},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.35.120}
}

@article{McMillan2,
  title = {Theoretical model of superconductivity and the martensitic transformation in $A15$ compounds},
  author = {Bilbro, Griff and McMillan, W. L.},
  journal = {Phys. Rev. B},
  volume = {14},
  issue = {5},
  pages = {1887--1892},
  numpages = {0},
  year = {1976},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.14.1887},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.14.1887}
}

%-----------------------Other TMDs Experiments ---------------

@article{CDWoldRev,
author = { J.A.   Wilson  and  A.D.   Yoffe },
title = {The transition metal dichalcogenides discussion and interpretation of the observed optical, electrical and structural properties},
journal = {Advances in Physics},
volume = {18},
number = {73},
pages = {193-335},
year  = {1969},
publisher = {Taylor & Francis},
doi = {10.1080/00018736900101307},
URL = {https://doi.org/10.1080/00018736900101307},
}

@Article{Arpes2HNbSe2,
author={Chatterjee, U.
and Zhao, J.
and Iavarone, M.
and Di Capua, R.
and Castellan, J. P.
and Karapetrov, G.
and Malliakas, C. D.
and Kanatzidis, M. G.
and Claus, H.
and Ruff, J. P. C.
and Weber, F.
and van Wezel, J.
and Campuzano, J. C.
and Osborn, R.
and Randeria, M.
and Trivedi, N.
and Norman, M. R.
and Rosenkranz, S.},
title={Emergence of coherence in the charge-density wave state of 2H-NbSe2},
journal={Nature Communications},
year={2015},
month={Feb},
day={17},
publisher={The Author(s) SN  -},
volume={6},
pages={6313 EP  -},
note={Article},
url={http://dx.doi.org/10.1038/ncomms7313}
}

@Article{SiposTaS2,
author={Sipos, B.
and Kusmartseva, A. F.
and Akrap, A.
and Berger, H.
and Forr{\'o}, L.
and Tutis, E.},
title={From Mott state to superconductivity in 1T-TaS2},
journal={Nature Materials},
year={2008},
month={Nov},
day={09},
publisher={Nature Publishing Group SN  -},
volume={7},
pages={960 EP  -},
note={Article},
url={http://dx.doi.org/10.1038/nmat2318}
}

@article{SedopTaSe2,
author = {Y. Liu and R. Ang and W. J. Lu and W. H. Song and L. J. Li and Y. P. Sun},
title = {Superconductivity induced by Se-doping in layered charge-density-wave system 1T-TaS2−xSex},
journal = {Applied Physics Letters},
volume = {102},
number = {19},
pages = {192602},
year = {2013},
doi = {10.1063/1.4805003},

URL = { 
        https://doi.org/10.1063/1.4805003
    
},
eprint = { 
        https://doi.org/10.1063/1.4805003
    
}
}

@article{SC2HTaSe2,
title = "Superconductivity in the quasi-two-dimensional conductor 2H-TaSe2",
journal = "Physica B: Condensed Matter",
volume = "284-288",
number = "Part 1",
pages = "551 - 552",
year = "2000",
issn = "0921-4526",
doi = "https://doi.org/10.1016/S0921-4526(99)02166-3",
url = "http://www.sciencedirect.com/science/article/pii/S0921452699021663",
author = "Ken-ichi Yokota and Gouo Kurata and Tomohiro Matsui and Hiroshi Fukuyama",
keywords = "Ac susceptibility, Charge density wave, Dichalcogenides, Layered material 2H-TaSe"
}

@article{SCinCuxTaSe2,
  title = {Tuning the charge density wave and superconductivity in ${\text{Cu}}_{x}{\text{TaS}}_{2}$},
  author = {Wagner, K. E. and Morosan, E. and Hor, Y. S. and Tao, J. and Zhu, Y. and Sanders, T. and McQueen, T. M. and Zandbergen, H. W. and Williams, A. J. and West, D. V. and Cava, R. J.},
  journal = {Phys. Rev. B},
  volume = {78},
  issue = {10},
  pages = {104520},
  numpages = {6},
  year = {2008},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.78.104520},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.78.104520}
}

@Article{Li2017,
author={Li, Lijun
and Deng, Xiaoyu
and Wang, Zhen
and Liu, Yu
and Abeykoon, Milinda
and Dooryhee, Eric
and Tomic, Aleksandra
and Huang, Yanan
and Warren, John B.
and Bozin, Emil S.
and Billinge, Simon J. L.
and Sun, Yuping
and Zhu, Yimei
and Kotliar, Gabriel
and Petrovic, Cedomir},
title={Superconducting order from disorder in 2H-TaSe{2-x}S_x},
journal={npj Quantum Materials},
year={2017},
volume={2},
number={1},
pages={11},
issn={2397-4648},
doi={10.1038/s41535-017-0016-9},
url={https://doi.org/10.1038/s41535-017-0016-9}
}

@article{Mutka83,
  title = {Superconductivity in irradiated charge-density-wave compounds $2H\ensuremath{-}\mathrm{Nb}{\mathrm{Se}}_{2}$, $2H\ensuremath{-}\mathrm{Ta}{\mathrm{S}}_{2}$, and $2H\ensuremath{-}\mathrm{Ta}{\mathrm{Se}}_{2}$},
  author = {Mutka, H.},
  journal = {Phys. Rev. B},
  volume = {28},
  issue = {5},
  pages = {2855--2858},
  numpages = {0},
  year = {1983},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.28.2855},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.28.2855}
}

%-----------------------SDW in Pnictides ----------------------
@article{ThSDWPnictides,
title = "Coexistence and competition of spin-density-wave and superconducting order parameters in iron-based superconductors",
journal = "Physics Letters A",
volume = "380",
number = "34",
pages = "2685 - 2692",
year = "2016",
issn = "0375-9601",
doi = "https://doi.org/10.1016/j.physleta.2016.06.005",
url = "http://www.sciencedirect.com/science/article/pii/S0375960116303103",
author = "Qing-Wei Wang and Da-Yong Liu and Ya-Min Quan and Liang-Jian Zou",
keywords = "Iron-base superconductor, Spin density wave, Orbital-selective competition, Singlet–triplet mixing"
}

@article{DemlerPRL,
  title = {Spin-Ordering Quantum Transitions of Superconductors in a Magnetic Field},
  author = {Demler, Eugene and Sachdev, Subir and Zhang, Ying},
  journal = {Phys. Rev. Lett.},
  volume = {87},
  issue = {6},
  pages = {067202},
  numpages = {4},
  year = {2001},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.87.067202},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.87.067202}
}


@article {Wang200,
	author = {Wang, Fa and Lee, Dung-Hai},
	title = {The Electron-Pairing Mechanism of Iron-Based Superconductors},
	volume = {332},
	number = {6026},
	pages = {200--204},
	year = {2011},
	doi = {10.1126/science.1200182},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/332/6026/200},
	eprint = {http://science.sciencemag.org/content/332/6026/200.full.pdf},
	journal = {Science}
}

@article{SchmiedtPair,
  title = {Superconducting pairing in the spin-density-wave phase of iron pnictides},
  author = {Schmiedt, Jacob and Brydon, P. M. R. and Timm, Carsten},
  journal = {Phys. Rev. B},
  volume = {89},
  issue = {5},
  pages = {054515},
  numpages = {13},
  year = {2014},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.054515},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.89.054515}
}

@article{GuPnictides,
  title = {Unified Phase Diagram for Iron-Based Superconductors},
  author = {Gu, Yanhong and Liu, Zhaoyu and Xie, Tao and Zhang, Wenliang and Gong, Dongliang and Hu, Ding and Ma, Xiaoyan and Li, Chunhong and Zhao, Lingxiao and Lin, Lifang and Xu, Zhuang and Tan, Guotai and Chen, Genfu and Meng, Zi Yang and Yang, Yi-feng and Luo, Huiqian and Li, Shiliang},
  journal = {Phys. Rev. Lett.},
  volume = {119},
  issue = {15},
  pages = {157001},
  numpages = {6},
  year = {2017},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.119.157001},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.157001}
}
@article{SiRev,
author={Si, Qimiao and Yu, Rong and Abrahams, Elihu},
Title ={High-temperature superconductivity in iron pnictides and chalcogenides},
journal={Nature Reviews Materials},
year ={2016},
month={March},
volume = {1},
pages  ={16017},
publisher={Macmillan Publishers Limited},
URL  ={http://dx.doi.org/10.1038/natrevmats.2016.17},
doi  ={10.1038/natrevmats.2016.17}
}

@article {Lake1759,
	author = {Lake, B. and Aeppli, G. and Clausen, K. N. and McMorrow, D. F. and Lefmann, K. and Hussey, N. E. and Mangkorntong, N. and Nohara, M. and Takagi, H. and Mason, T. E. and Schr{\"o}der, A.},
	title = {Spins in the Vortices of a High-Temperature Superconductor},
	volume = {291},
	number = {5509},
	pages = {1759--1762},
	year = {2001},
	doi = {10.1126/science.1056986},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/291/5509/1759},
	eprint = {http://science.sciencemag.org/content/291/5509/1759.full.pdf},
	journal = {Science}
}


%-----------------------Experiments for CDW in HTSc------------
@Article{Wise2008,
author={Wise, W. D.
and Boyer, M. C.
and Chatterjee, Kamalesh
and Kondo, Takeshi
and Takeuchi, T.
and Ikuta, H.
and Wang, Yayu
and Hudson, E. W.},
title={Charge-density-wave origin of cuprate checkerboard visualized by scanning tunnelling microscopy},
journal={Nature Physics},
year={2008},
month={Jul},
day={06},
publisher={Nature Publishing Group SN  -},
volume={4},
pages={696 EP  -},
url={http://dx.doi.org/10.1038/nphys1021}
}

@article{tJStripe,
  title = {Competing States in the $t$-$J$ Model: Uniform $d$-Wave State versus Stripe State},
  author = {Corboz, Philippe and Rice, T. M. and Troyer, Matthias},
  journal = {Phys. Rev. Lett.},
  volume = {113},
  issue = {4},
  pages = {046402},
  numpages = {5},
  year = {2014},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.113.046402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.113.046402}
}


@Article{Chang2012,
author={Chang, J.
and Blackburn, E.
and Holmes, A. T.
and Christensen, N. B.
and Larsen, J.
and Mesot, J.
and Liang, Ruixing
and Bonn, D. A.
and Hardy, W. N.
and Watenphul, A.
and Zimmermann, M. v.
and Forgan, E. M.
and Hayden, S. M.},
title={Direct observation of competition between superconductivity and charge density wave order in $YBa_2Cu_3O_{6.67}$},
journal={Nature Physics},
year={2012},
month={Oct},
day={14},
publisher={Nature Publishing Group SN  -},
volume={8},
pages={871 EP  -},
url={http://dx.doi.org/10.1038/nphys2456}
}

@article{CupratesPRB,
  title = {Direct observation of charge order in underdoped and optimally doped ${\mathrm{Bi}}_{2}{(\mathrm{Sr},\mathrm{La})}_{2}{\mathrm{CuO}}_{6+\ensuremath{\delta}}$ by resonant inelastic x-ray scattering},
  author = {Peng, Y. Y. and Salluzzo, M. and Sun, X. and Ponti, A. and Betto, D. and Ferretti, A. M. and Fumagalli, F. and Kummer, K. and Le Tacon, M. and Zhou, X. J. and Brookes, N. B. and Braicovich, L. and Ghiringhelli, G.},
  journal = {Phys. Rev. B},
  volume = {94},
  issue = {18},
  pages = {184511},
  numpages = {8},
  year = {2016},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.94.184511},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.94.184511}
}

@Article{Hashimoto2014,
author={Hashimoto, Makoto
and Vishik, Inna M.
and He, Rui-Hua
and Devereaux, Thomas P.
and Shen, Zhi-Xun},
title={Energy gaps in high-transition-temperature cuprate superconductors},
journal={Nature Physics},
year={2014},
month={Jun},
day={30},
publisher={Nature Publishing Group SN  -},
volume={10},
pages={483 EP  -},
note={Review Article},
url={http://dx.doi.org/10.1038/nphys3009}
}

@Article{DisorderCDWHTSc,
author={Campi, G.
and Bianconi, A.
and Poccia, N.
and Bianconi, G.
and Barba, L.
and Arrighetti, G.
and Innocenti, D.
and Karpinski, J.
and Zhigadlo, N. D.
and Kazakov, S. M.
and Burghammer, M.
and Zimmermann, M. v.
and Sprung, M.
and Ricci, A.},
title={Inhomogeneity of charge-density-wave order and quenched disorder in a high-Tc superconductor},
journal={Nature},
year={2015},
month={Sep},
day={16},
publisher={Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved. SN  -},
volume={525},
pages={359 EP  -},
url={http://dx.doi.org/10.1038/nature14987}
}

@article{silvaNeto2014,
	author = {da Silva Neto, Eduardo H. and Aynajian, Pegor and Frano, Alex and Comin, Riccardo and Schierle, Enrico and Weschke, Eugen and Gyenis, Andr{\'a}s and Wen, Jinsheng and Schneeloch, John and Xu, Zhijun and Ono, Shimpei and Gu, Genda and Le Tacon, Mathieu and Yazdani, Ali},
	title = {Ubiquitous Interplay Between Charge Ordering and High-Temperature Superconductivity in Cuprates},
	volume = {343},
	number = {6169},
	pages = {393--396},
	year = {2014},
	doi = {10.1126/science.1243479},
	publisher = {American Association for the Advancement of Science},
	issn = {0036-8075},
	URL = {http://science.sciencemag.org/content/343/6169/393},
	eprint = {http://science.sciencemag.org/content/343/6169/393.full.pdf},
	journal = {Science}
}

@article{Croft2014,
  title = {Charge density wave fluctuations in ${\text{La}}_{2\ensuremath{-}x}$${\text{Sr}}_{x}$${\text{CuO}}_{4}$ and their competition with superconductivity},
  author = {Croft, T. P. and Lester, C. and Senn, M. S. and Bombardi, A. and Hayden, S. M.},
  journal = {Phys. Rev. B},
  volume = {89},
  issue = {22},
  pages = {224513},
  numpages = {8},
  year = {2014},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.89.224513},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.89.224513}
}

@article {Mesaros,
	author = {Mesaros, Andrej and Fujita, Kazuhiro and Edkins, Stephen D. and Hamidian, Mohammad H. and Eisaki, Hiroshi and Uchida, Shin-ichi and Davis, J. C. S{\'e}amus and Lawler, Michael J. and Kim, Eun-Ah},
	title = {Commensurate 4a0-period charge density modulations throughout the Bi2Sr2CaCu2O8+x pseudogap regime},
	volume = {113},
	number = {45},
	pages = {12661--12666},
	year = {2016},
	doi = {10.1073/pnas.1614247113},
	publisher = {National Academy of Sciences},
	abstract = {},
	issn = {0027-8424},
	URL = {http://www.pnas.org/content/113/45/12661},
	eprint = {http://www.pnas.org/content/113/45/12661.full.pdf},
	journal = {Proceedings of the National Academy of Sciences}
}

%------------------------Theory Attr. Hubb Model---------------------------------

@article{PhaseAHM,
  title = {Phase diagram of the two-dimensional negative-U Hubbard model},
  author = {Scalettar, R. T. and Loh, E. Y. and Gubernatis, J. E. and Moreo, A. and White, S. R. and Scalapino, D. J. and Sugar, R. L. and Dagotto, E.},
  journal = {Phys. Rev. Lett.},
  volume = {62},
  issue = {12},
  pages = {1407--1410},
  numpages = {0},
  year = {1989},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.62.1407},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.62.1407}
}

@article{GTR,
  title = {Role of Spatial Amplitude Fluctuations in Highly Disordered $\mathit{s}$-Wave Superconductors},
  author = {Ghosal, Amit and Randeria, Mohit and Trivedi, Nandini},
  journal = {Phys. Rev. Lett.},
  volume = {81},
  issue = {18},
  pages = {3940--3943},
  numpages = {0},
  year = {1998},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.81.3940},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.81.3940}
}

@article{Moreo,
  title = {Two-dimensional negative-U Hubbard model},
  author = {Moreo, A. and Scalapino, D. J.},
  journal = {Phys. Rev. Lett.},
  volume = {66},
  issue = {7},
  pages = {946--948},
  numpages = {0},
  year = {1991},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.66.946},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.66.946}
}

@article{RTS,
  title = {Effect of disorder on charge-density wave and superconducting order in the half-filled attractive Hubbard model},
  author = {Huscroft, C. and Scalettar, R. T.},
  journal = {Phys. Rev. B},
  volume = {55},
  issue = {2},
  pages = {1185--1193},
  numpages = {0},
  year = {1997},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.55.1185},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.55.1185}
}

@article{Miller,
  title     = "On the Coexistence of Superconductivity and Charge Density Waves",
  author    = "P Miller and B Janko and BL Gyorffy",
  year      = "1993",
  volume    = "210",
  pages     = "343 -- 349",
  journal   = "Physica C: Superconductivity and its Applications",
  issn      = "0921-4534",
  publisher = "Elsevier",
}
@article{DosSantos,
  title = {Second-neighbor hopping in the attractive Hubbard model},
  author = {dos Santos, Raimundo R.},
  journal = {Phys. Rev. B},
  volume = {46},
  issue = {9},
  pages = {5496--5498},
  numpages = {0},
  year = {1992},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.46.5496},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.46.5496}
}


@article{Balsiero,
  title = {Superconductivity and charge-density waves},
  author = {Balseiro, C. A. and Falicov, L. M.},
  journal = {Phys. Rev. B},
  volume = {20},
  issue = {11},
  pages = {4457--4464},
  numpages = {0},
  year = {1979},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.20.4457},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.20.4457}
}


@article{MicnasRMP,
  title = {Superconductivity in narrow-band systems with local nonretarded attractive interactions},
  author = {Micnas, R. and Ranninger, J. and Robaszkiewicz, S.},
  journal = {Rev. Mod. Phys.},
  volume = {62},
  issue = {1},
  pages = {113--171},
  numpages = {0},
  year = {1990},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.62.113},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.62.113}
}

@article{Micnasdis,
title = "Charge ordering and superconductivity in bipolaronic systems with diagonal disorder",
journal = "Physica A: Statistical Mechanics and its Applications",
volume = "131",
number = "2",
pages = "393 - 409",
year = "1985",
issn = "0378-4371",
doi = "https://doi.org/10.1016/0378-4371(85)90005-6",
url = "http://www.sciencedirect.com/science/article/pii/0378437185900056",
author = "R. Micnas and S. Robaszkiewicz and K.A. Chao"
}

@article{Robdis,
title = "Effects of diagonal disorder on charge density wave and superconductivity in local pair systems",
journal = "Physica A: Statistical Mechanics and its Applications",
volume = "299",
number = "3",
pages = "475 - 493",
year = "2001",
issn = "0378-4371",
doi = "https://doi.org/10.1016/S0378-4371(01)00261-8",
url = "http://www.sciencedirect.com/science/article/pii/S0378437101002618",
author = "Grzegorz Pawłowski and Stanisław Robaszkiewicz",
keywords = "Hard-core bosons, Local electron pairing (local pairs), Disordered systems, Charge density waves, Superconductivity, Phase separations"
}

@article{SUN,
  title = {Disorder-induced charge-density-wave\char21{}superfluid transition in $\mathrm{SU}(N)$ Fermi systems},
  author = {Sakaida, Masaru and Kawakami, Norio},
  journal = {Phys. Rev. A},
  volume = {90},
  issue = {1},
  pages = {013632},
  numpages = {8},
  year = {2014},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.90.013632},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.90.013632}
}

@article{ModBroyd,
  title = {Modified Broyden's method for accelerating convergence in self-consistent calculations},
  author = {Johnson, D. D.},
  journal = {Phys. Rev. B},
  volume = {38},
  issue = {18},
  pages = {12807--12813},
  numpages = {0},
  year = {1988},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.38.12807},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.38.12807}
}

@article{Kalinsky,
  title = {Competition of superconductivity and antiferromagnetism in a d-wave vortex lattice},
  author = {Ghosal, Amit and Kallin, Catherine and Berlinsky, A. John},
  journal = {Phys. Rev. B},
  volume = {66},
  issue = {21},
  pages = {214502},
  numpages = {10},
  year = {2002},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.66.214502},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.66.214502}
}

@article{Debmalya1,
  author={Debmalya Chakraborty and Amit Ghosal},
  title={Effects of strong disorder in strongly correlated superconductors},
  journal={Physical Review B},
  volume={95},
  number={1},
  pages={},
  url={http://dx.doi.org/10.1103/PhysRevB.95.014516},
  year={2017},
  abstract={}
}


  	
@article{Debmalya0,
  author={Debmalya Chakraborty and Amit Ghosal},
  title={Fate of disorder-induced inhomogeneities in strongly correlated d-wave superconductors},
  journal={New Journal of Physics},
  volume={16},
  number={10},
  pages={103018},
  url={http://stacks.iop.org/1367-2630/16/i=10/a=103018},
  year={2014},
  abstract={W}
}

